Efficient Verification of Multi-Property Designs (The Benefit of Wrong Assumptions) (Extended Version)

We consider the problem of efficiently checking a set of safety properties P1,....,Pk of one design. We introduce a new approach called JA-verification where JA stands for "Just-Assume" (as opposed to "assume-guarantee"). In this approach, when proving property Pi, one assumes that every property Pj for j!=i holds. The process of proving properties either results in showing that P1,....,Pk hold without any assumptions or finding a "debugging set" of properties. The latter identifies a subset of failed properties that cause failure of other properties. The design behaviors that cause the properties in the debugging set to fail must be fixed first. Importantly, in our approach, there is no need to prove the assumptions used. We describe the theory behind our approach and report experimental results that demonstrate substantial gains in performance, especially in the cases where a small debugging set exists.

==> todo <==
=========================

        T O  D O

=========================




=========================

      D O N E

=========================
*) put together a version to start with
*) correct Proposition~\ref{prop:lg_proofs}
*) correct Proposition~\ref{prop:joint_sep}
*) review the proofs
*) modify the subsection of clause re-using
*) add explanation of lifting in IC3
*) mention importance of lifting in ic3-db
*) remove references to the technical
   report
*) modify the beginning of the
   experimental section
*) write subsection with designs having
   many properties
*) add time limit per property
   for the table reporting results
   on designs with large number of properties
*) write a section relating global and  local proofs
*) write subsection on local and
   global proofs in the second experimental section
*) write the subsection on relation between
   lifting and separate verification=
*) write the second experimental section   
*) modify the first experimental section
